Machine Learning Interventions for Weed Detection using Multispectral Imagery and Unmanned Aerial Vehicles -- A Systematic Review

The growth of weeds poses a significant challenge to agricultural productivity, necessitating efficient and accurate weed detection and management strategies. The combination of multispectral imaging and drone technology has emerged as a promising approach to tackle this issue, enabling rapid and cost-effective monitoring of large agricultural fields. This systematic review surveys and evaluates the state-of-the-art in machine learning interventions for weed detection that utilize multispectral images captured by unmanned aerial vehicles. The study describes the various models used for training, features extracted from multi-spectral data, their efficiency and effect on the results, the performance analysis parameters, and also the current challenges faced by researchers in this domain. The review was conducted in accordance with the PRISMA guidelines. Three sources were used to obtain the relevant material, and the screening and data extraction were done on the COVIDENCE platform. The search string resulted in 600 papers from all sources. The review also provides insights into potential research directions and opportunities for further advancements in the field. These insights would serve as a valuable guide for researchers, agricultural scientists, and practitioners in developing precise and sustainable weed management strategies to enhance agricultural productivity and minimize ecological impact.

==> backuo.tex <==
% \bibliographystyle{apa}
% \bibliography{sample}

% [1]. Alexandridis, Thomas K., Afroditi Alexandra Tamouridou, Xanthoula Eirini Pantazi, Anastasia L. Lagopodi, Javid Kashefi, Georgios Ovakoglou, Vassilios Polychronos, and Dimitrios Moshou. 2017 Sept. 1. “Novelty Detection Classifiers in Weed Mapping: Silybum marianum Detection on UAV Multispectral Images.” \emph{Sensors} 17, no. 9: 2007. https://doi.org/10.3390/s17092007, PubMed: 28862663, PubMed Central: PMC5621143..

% [2].  Amarasingam, N., M. Hamilton, J. E. Kelly, L. Zheng, J. Sandino, F. Gonzalez, R. L. Dehaan, and H. Cherry. 2023. “Autonomous Detection of Mouse-Ear Hawkweed Using Drones, Multispectral Imagery and Supervised Machine Learning.” \emph{Remote Sensing} 15, no. 6: 1633. https://doi.org/10.3390/rs15061633.

% [3]. Naveed, A., W. Muhammad, M. J. Irshad, M. J. Aslam, S. M. Manzoor, T. Kausar, and Y. Lu. 2023. “Saliency-Based Semantic Weeds Detection and Classification Using UAV Multispectral Imaging.” In \emph{IEEE Access} 11: 11991–2003. https://doi.org/10.1109/ACCESS.2023.3242604.

% [4].  Bento, Nicole Lopes, Gabriel Araújo e Silva Ferraz, Jhones da Silva Amorim, Lucas Santos Santana, Rafael Alexandre Pena Barata, Daniel Veiga Soares, and Patrícia Ferreira Ponciano Ferraz. 2023. "Weed Detection and Mapping of a Coffee Farm by a Remotely Piloted Aircraft System" \textit{Agronomy} 13, no. 3: 830. https://doi.org/10.3390/agronomy13030830 

% [5]. Che’Ya, N. N., E. Dunwoody, and M. Gupta. 2021. “Assessment of Weed Classification Using Hyperspectral Reflectance and Optimal Multispectral UAV Imagery.” \emph{Agronomy} 11, no. 7: 1435. https://doi.org/10.3390/agronomy11071435.

% [6].  De Castro, A. I., J. Torres-Sánchez, J. M. Peña, F. M. Jiménez-Brenes, O. Csillik, and F. López-Granados. 2018. “An Automatic Random Forest-OBIA Algorithm for Early Weed Mapping Between and Within Crop Rows Using UAV Imagery.” \emph{Remote Sensing} 10, no. 3: 285. https://doi.org/10.3390/rs10020285.

% [7]. Kerdegari, H., M. Razaak, V. Argyriou, and P. Remagnino. 2019. “Smart Monitoring of Crops Using Generative Adversarial Networks.” In \emph{Lecture Notes in Computer Science}. CAIP 2019, edited by M. Vento, and G. Percannella Computer Analysis of Images and Patterns(), vol 11678. Springer, Cham. https://doi.org/10.1007/978-3-030-29888-3\_45.

% [8]. Bah, M. D., A. Hafiane, R. Canals, and B. Emile. 2019. “Deep Features and One-Class Classification with Unsupervised Data for Weed Detection in UAV Images.” \emph{Ninth International Conference on Image Processing Theory, Tools and Applications (IPTA)} vol. 2019: 1–5. \href{https://doi.org/10.1109/IPTA.2019.8936091}{https://doi.org/10.1109/IPTA.2019.8936091} 

% [9]. Fraccaro, P., J. Butt, B. Edwards, R. P. Freckleton, D. Z. Childs, K. Reusch, and D. Comont. 2022. “A Deep Learning Application to Map Weed Spatial Extent from Unmanned Aerial Vehicles Imagery.” \textit{Remote Sensing} 14, no. 17: 4197. \href{https://doi.org/10.3390/rs14174197}{https://doi.org/10.3390/rs14174197}. 

% [10]. Khoshboresh-Masouleh, M., and R. Shah-Hosseini. 2022. “Uncertainty Estimation in Deep Meta-Learning for Crop and Weed Detection from Multispectral UAV Images.” \textit{IEEE Mediterranean and Middle East. Geoscience and Remote Sensing Symposium (M2GARSS)}, Istanbul, Turkey vol. 2022: 165–8. \href{https://doi.org/10.1109/m2garss52314.2022.9839758}{https://doi.org/10.1109/M2GARSS52314.2022.9839758}. 

% [11]. Pérez-Ortiz, M., P. A. Gutiérrez, J. M. Peña, J. Torres-Sánchez, F. López-Granados, and C. Hervás-Martínez. 2016. “Machine Learning Paradigms for Weed Mapping via Unmanned Aerial Vehicles.” \emph{IEEE Symposium Series on Computational Intelligence (SSCI)}, Athens, Greece 2016: 1–8. \href{https://doi.org/10.1109/ssci.2016.7849987}{https://doi.org/10.1109/SSCI.2016.7849987}. 

% [12]. Papp, L., B. van Leeuwen, P. Szilassi, Z. Tobak, J. Szatmári, M. Árvai, J. Mészáros, and L. Pásztor. 2021. “Monitoring Invasive Plant Species Using Hyperspectral Remote Sensing Data.” \textit{Land} 10, no. 1: 29. \href{https://doi.org/10.3390/land10010029}{https://doi.org/10.3390/land10010029}. 

% [13]. Pérez-Ortiz, M., J. M. Peña, P. A. Gutiérrez, J. Torres-Sánchez, C. Hervás-Martínez, and F. López-Granados. 2015. “A Semi-supervised System for Weed Mapping in Sunflower Crops Using Unmanned Aerial Vehicles and a Crop Row Detection Method.” \textit{Applied Soft Computing} 37: 533–44. \href{https://doi.org/10.1016/j.asoc.2015.08.027}{https://doi.org/10.1016/j.asoc.2015.08.027}. 

% [14]. Sa, I., M. Popović, R. Khanna, Z. Chen, P. Lottes, F. Liebisch, J. Nieto, C. Stachniss, A. Walter, and R. Siegwart. 2018. “WeedMap: A Large-Scale Semantic Weed Mapping Framework Using Aerial Multispectral Imaging and Deep Neural Network for Precision Farming.” \textit{Remote Sensing} 10, no. 9: 1423. \href{https://doi.org/10.3390/rs10091423}{https://doi.org/10.3390/rs10091423}. 

% [15].  Sanders, J. T., E. A. L. Jones, R. Austin, G. T. Roberson, R. J. Richardson, and W. J. Everman. 2021. “Remote Sensing for Palmer Amaranth (Amaranthus palmeri S. Wats.) Detection in Soybean (Glycine max (L.) Merr.).” \textit{Agronomy} 11, no. 10: 1909. \href{https://doi.org/10.3390/agronomy11101909}{https://doi.org/10.3390/agronomy11101909}. 

% [16]. Scherrer, Bryan, John Sheppard, Prashant Jha, and Joseph A. Shaw. 2019. “Hyperspectral Imaging and Neural Networks to Classify Herbicide-Resistant Weeds.” \textit{Journal of Applied Remote Sensing} 13, no. 4: 044516. \href{https://doi.org/10.1117/1.jrs.13.044516}{https://doi.org/10.1117/1.JRS.13.044516}. 

% [17]. Moazzam, S. I., U. S. Khan, T. Nawaz, and W. S. Qureshi. 2022. “Crop and Weeds Classification in Aerial Imagery of Sesame Crop Fields Using a Patch-Based Deep Learning Model-Ensembling Method.” 2nd \emph{International Conference on Digital Futures and Transformative Technologies (ICoDT2)}, Rawalpindi, Pakistan vol. 2022: 1–7. \href{https://doi.org/10.1109/icodt255437.2022.9787455}{https://doi.org/10.1109/ICoDT255437.2022.9787455}. 

% [18]. Su, Jinya, Dewei Yi, Matthew Coombes, Cunjia Liu, Xiaojun Zhai, Klaus McDonald-Maier, and W. Chen. 2022. “Spectral Analysis and Mapping of Blackgrass Weed by Leveraging Machine Learning and UAV Multispectral Imagery.” \textit{Computers \& Electronics in Agriculture} 192: 106621. \href{https://doi.org/10.1016/j.compag.2021.106621}{https://doi.org/10.1016/j.compag.2021.106621}. 

% [19]. Tamouridou, A. A., T. K. Alexandridis, X. E. Pantazi, A. L. Lagopodi, J. Kashefi, and D. Moshou. 2017. “Evaluation of UAV Imagery for Mapping Silybum marianum Weed Patches.” \textit{International Journal of Remote Sensing} 38, no. 8–10 (20 April - 20 May 2017): 2246–59. \href{https://doi.org/10.1080/01431161.2016.1252475}{https://doi.org/10.1080/01431161.2016.1252475}. 

% [20]. Wang, Shubo, Y. Han, Jian Chen, Xiongkui He, Zichao Zhang, Xuzan Liu, and Kai Zhang. 2021. “Weed Density Extraction Based on Few-Shot Learning Through UAV Remote Sensing RGB and Multispectral Images in Ecological Irrigation Area.” \textit{Frontiers in Plant Science} 12: 735230. \href{https://doi.org/10.3389/fpls.2021.735230}{https://doi.org/10.3389/fpls.2021.735230}, PubMed: \href{http://www.ncbi.nlm.nih.gov/pubmed/35399196}{35399196}, PubMed Central: \href{https://www.ncbi.nlm.nih.gov/pmc/articles/PMC8987725}{PMC8987725}. 

% [21]. Zisi, T., T. K. Alexandridis, S. Kaplanis, I. Navrozidis, A.-A. Tamouridou, A. Lagopodi, D. Moshou, and V. Polychronos. 2018. “Incorporating Surface Elevation Information in UAV Multispectral Images for Mapping Weed Patches.” \textit{Journal of Imaging} 4, no. 11: 132. \href{https://doi.org/10.3390/jimaging4110132}{https://doi.org/10.3390/jimaging4110132}. 

% [22]. Murad, Nafeesa Yousuf, Tariq Mahmood, Abdur Rahim Mohammad Forkan, Ahsan Morshed, Prem Prakash Jayaraman, and Muhammad Shoaib Siddiqui. 2023 Mar. 31. “Weed Detection Using Deep Learning: A Systematic Literature Review.” \textit{Sensors} 23, no. 7: 3670. \href{https://doi.org/10.3390/s23073670}{https://doi.org/10.3390/s23073670}, PubMed: \href{http://www.ncbi.nlm.nih.gov/pubmed/37050730}{37050730}, PubMed Central: \href{https://www.ncbi.nlm.nih.gov/pmc/articles/PMC10098587}{PMC10098587}. 

% [23]. Rejeb, A., A. Abdollahi, K. Rejeb, and H. Treiblmaier. 2022. “Drones in Agriculture: A Review and Bibliometric Analysis.” \textit{Computers \& Electronics in Agriculture} 198: 107017. \href{https://doi.org/10.1016/j.compag.2022.107017}{https://doi.org/10.1016/j.compag.2022.107017}. 

% [24]. Yang, Guijun, Jiangang Liu, Chunjiang Zhao, Zhenhong Li, Yanbo Huang, Haiyang Yu, B. Xu, Xiaodong Yang, Dongmei Zhu, Xiaoyan Zhang, Ruyang Zhang, Haikuan Feng, Xiaoqing Zhao, Zhenhai Li, Heli Li, and Hao Yang. 2017 Jun. 30. “Unmanned Aerial Vehicle Remote Sensing for Field-Based Crop Phenotyping: Current Status and Perspectives.” \textit{Frontiers in Plant Science} 8: 1111. \href{https://doi.org/10.3389/fpls.2017.01111}{https://doi.org/10.3389/fpls.2017.01111}, PubMed: \href{http://www.ncbi.nlm.nih.gov/pubmed/28713402}{28713402}, PubMed Central: \href{https://www.ncbi.nlm.nih.gov/pmc/articles/PMC5492853}{PMC5492853}. 

% [25]. Mohidem, N. A., N. N. Che’Ya, A. S. Juraimi, W. F. Fazlil Ilahi, M. H. Mohd Roslim, N. Sulaiman, M. Saberioon, and N. Mohd Noor. 2021. “How Can Unmanned Aerial Vehicles Be Used for Detecting Weeds in Agricultural Fields?.” \textit{Agriculture} 11, no. 10: 1004. \href{https://doi.org/10.3390/agriculture11101004}{https://doi.org/10.3390/agriculture11101004}. 

% [26]. Moher, David, Alessandro Liberati, Jennifer Tetzlaff, Douglas G. Altman, and PRISMA Group. 2009 Jul. 21. “Preferred Reporting Items for Systematic Reviews and Meta-Analyses: the PRISMA Statement.” \textit{PLOS Medicine} 6, no. 7: e1000097. \href{https://doi.org/10.1371/journal.pmed.1000097}{https://doi.org/10.1371/journal.pmed.1000097}. Epub July 21 2009. PubMed: \href{http://www.ncbi.nlm.nih.gov/pubmed/19621072}{19621072}, PubMed Central: \href{https://www.ncbi.nlm.nih.gov/pmc/articles/PMC2707599}{PMC2707599}. 

% [27].  Moher, David, Alessandro Liberati, Jennifer Tetzlaff, Douglas G. Altman, and PRISMA Group. 2009. “Preferred Reporting Items for Systematic Reviews and Meta-Analyses: the PRISMA Statement.” \textit{PLOS Medicine} 6, no. 7: e1000097. \href{https://doi.org/10.1371/journal.pmed.1000097}{https://doi.org/10.1371/journal.pmed.1000097}. 

% [28]. Sulaiman, N., N. N. Che’Ya, M. H. Mohd Roslim, A. S. Juraimi, N. Mohd Noor, and W. F. Fazlil Ilahi. 2022. “The Application of Hyperspectral Remote Sensing Imagery (HRSI) for Weed Detection Analysis in Rice Fields: A Review.” \textit{Applied Sciences} 12, no. 5: 2570. \href{https://doi.org/10.3390/app12052570}{https://doi.org/10.3390/app12052570}. 

% [29].Su, Wen-Hao, and Da-Wen Sun. 2018 Jan. “Multispectral Imaging for Plant Food Quality Analysis and Visualization” \textit{Comprehensive Reviews in Food Science \& Food Safety} 17, no. 1: 220–39. \href{https://doi.org/10.1111/1541-4337.12317}{https://doi.org/10.1111/1541-4337.12317}, PubMed: \href{http://www.ncbi.nlm.nih.gov/pubmed/33350065}{33350065}. 

% [30].Laliberte, A. S., and A. Rango. 2009. “Texture and Scale in Object-Based Analysis of Subdecimeter Resolution Unmanned Aerial Vehicle (UAV) Imagery.” \textit{IEEE Transactions on Geoscience \& Remote Sensing} 47, no. 3: 761–70. \href{https://doi.org/10.1109/TGRS.2008.2009355}{https://doi.org/10.1109/TGRS.2008.2009355}. 

% [31]. Gupta, C., A. S. Suggala, A. Goyal, H. V. Simhadri, B. Paranjape, A. J. Kumar, S. Goyal, R. Udupa, M. Varma, and P. Jain. 2017. “ProtoNN: Compressed and Accurate kNN for Resource-Scarce Devices.” \emph{International Conference on Machine Learning.}

% [32]. Pimentel, D., R. Zuniga, and D. Morrison. 2005. “Update on the Environmental and Economic Costs Associated with Alien-Invasive Species in the United States.” \textit{Ecological Economics} 52, no. 3: 273–88. \href{https://doi.org/10.1016/j.ecolecon.2004.10.002}{https://doi.org/10.1016/j.ecolecon.2004.10.002}. 

% [33]. Kubiak, A., A. Wolna-Maruwka, A. Niewiadomska, and A. A. Pilarska. 2022. “The Problem of Weed Infestation of Agricultural Plantations vs. the Assumptions of the European Biodiversity Strategy.” \textit{Agronomy} 12, no. 8: 1808. \href{https://doi.org/10.3390/agronomy12081808}{https://doi.org/10.3390/agronomy12081808}. 

% [34]. European Commission. 2020. “Communication from the Commission to the European Parliament, the Council, the European Economic and Social Committee, and The Committee of the Regions, EU Biodiversity Strategy for 2030, Bringing Nature Back into Our Lives”. https://eur-lex.europa.eu/legal-content/EN/TXT/?uri=CELEX:52020DC0380. Brussels, Belgium: European Commission. 

% [35]. European Commission. 2020. “Communication from the Commission to the European Parliament, the European Council, the Council, the European Economic and Social Committee, and The Committee of the Regions, Farm to Fork Strategy for a Fair, Healthy, and Environmentally Friendly Food System." https://eur-lex.europa.eu/legal-content/EN/TXT/?uri=CELEX\%3A52020DC0381. Brussels, Belgium: European Commission. 

% [36] Woyessa, D., "Weed Control Methods Used in Agriculture" \emph{American Journal of Life Science and Innovation} 2022. 1:19-26. doi: 10.54536/ajlsi.v1i1.413. 

% [37] Rao, A.N., Ravi Gopal Singh, Gulshan Mahajan, and S.P. Wani "Weed research issues, challenges, and opportunities in India" \emph{Crop Protection}, Volume 134, 2020, 104451, ISSN 0261-2194. https://doi.org/10.1016/j.cropro.2018.02.003.

% [38] FAO (Food and Agriculture Organization of the United Nations). https://www.fao.org/home/en/.

% [39] Khan, Nawab, Ram L. Ray, Ghulam Raza Sargani, Muhammad Ihtisham, Muhammad Khayyam, and Sohaib Ismail. 2021. "Current Progress and Future Prospects of Agriculture Technology: Gateway to Sustainable Agriculture" \emph{Sustainability} 13, no. 9: 4883. https://doi.org/10.3390/su13094883

% [40] Thilakarathne, Navod Neranjan, Muhammad Saifullah Abu Bakar, Pg Emerolylariffion Abas, and Hayati Yassin. 2022. "A Cloud Enabled Crop Recommendation Platform for Machine Learning-Driven Precision Farming" \emph{Sensors} 22, no. 16: 6299. https://doi.org/10.3390/s22166299

% [41] Braga, A. F., L. A. Chiconi, A. L. Bacha, G. Teixeira, L. C. Cunha Junior, and P. LdC. A. Alves. 2023. “Discrimination of Morningglory Species (Ipomoea spp.) Using Near-Infrared Spectroscopy and Multivariate Analysis.” \emph{Weed Science} 71, no. 2: 104–11. https://doi.org/10.1017/wsc.2023.6.

% [42] Esposito, M., M. Crimaldi, V. Cirillo, F. Sarghini, and A. Maggio. 2021. “Drone and Sensor Technology for Sustainable Weed Management: A Review.” \emph{Chemical & Biological Technologies in Agriculture} 8, no. 1. https://doi.org/10.1186/s40538-021-00217-8.

% [43] Smith, J. D., T. Dubois, R. Mallogo, E.-F. Njau, S. Tua, and R. Srinivasan, hosts range of the invasive tomato pest tuta absoluta meyrick (Lepidoptera: Gelechiidae) on solanaceous crops and weeds in Tanzania" \emph{Florida Entomological Society}. 2019. http://www.jstor.org/stable/26567447 vol. 101, no. 4: 573–9.

% [44] Roshan, P., A. Kulshreshtha, and V. Hallan "Global Weed-Infecting Geminiviruses BT-Geminiviruses: Impact, Challenges and Approaches" \emph{Berlin: Springer}. 2019: 103–21. https://doi.org/10.1007/978-3-030-18248-9\_6

% [45] Rango, A., A. Laliberte, J. E. Herrick, C. Winters, K. Havstad, and C. Steele. 2009. “Unmanned Aerial Vehicle-Based Remote Sensing for Rangeland Assessment, Monitoring, and Management.” \emph{Journal of Applied Remote Sensing 3}, no. 1: 033542. https://doi.org/10.1117/1.3216822


% [46] Viana, C. M., S. Oliveira, S. C. Oliveira, J. Rocha, "Land Use, and Land Cover Change" 2019 \emph{Detection and Urban Sprawl Analysis Elsevier: 621–51} https://doi.org/10.1016/B978-0-12-815226-3.00029-6.


% [47] Woebbecke, D. M., G. E. Meyer, K. Von Bargen, and D. A. Mortensen. 1995. “Color Indices for Weed Identification Under Various Soil, Residue, and Lighting Conditions.” \emph{Transactions of the ASAE. American Society of Agricultural Engineers} 38: 259–69. https://doi.org/10.13031/2013.27838.


% [48] Yeom, J., J. Jung, A. Chang, A. Ashapure, M. Maeda, A. Maeda, and J. Landivar. 2019. “Comparison of Vegetation Indices Derived from UAV Data for Differentiation of Tillage Effects in Agriculture.” \emph{Remote Sensing} 11, no. 13: 1548. https://doi.org/10.3390/rs11131548.


% [49] Skjelvareid, Martin, Katalin Blix, Galice Guillaume Hoarau, Eli Rinde, and Kasper Hancke "Mapping seagrass and rockweed habitats using UAV hyperspectral imaging and machine learning" \emph{Marine Geological and Biological Habitat Mapping Conference} 2023

% [50] Deng, Lei, Yanan Yan, Huili Gong, Fuzhou Duan, and Ruofei Zhong, "The effect of spatial resolution on radiometric and geometric performances of a UAV-mounted hyperspectral 2D imager" \emph{ISPRS Journal of Photogrammetry and Remote Sensing} Volume 144, 2018, Pages 298-314, ISSN 0924-2716. https://doi.org/10.1016/j.isprsjprs.2018.08.002.

% [51] Moazzam, S.I., U. S. Khan, T. Nawaz, and W. S. Qureshi, "Crop and Weeds Classification in Aerial Imagery of Sesame Crop Fields Using a Patch-Based Deep Learning Model-Ensembling Method," \emph{2022 2nd International Conference on Digital Futures and Transformative Technologies (ICoDT2)}, Rawalpindi, Pakistan, 2022, pp. 1-7. doi: 10.1109/ICoDT255437.2022.9787455.5.

% [52] Mesas-Carrascosa, Francisco-Javier, Jorge Torres-Sánchez, Inmaculada Clavero-Rumbao, Alfonso García-Ferrer, Jose-Manuel Peña, Irene Borra-Serrano, and Francisca López-Granados. 2015. "Assessing Optimal Flight Parameters for Generating Accurate Multispectral Orthomosaicks by UAV to Support Site-Specific Crop Management" \emph{Remote Sensing} 7, no. 10: 12793-12814 https://doi.org/10.3390/rs71012793.

